Prompt Sketching for Large Language Models

Many recent prompting strategies for large language models (LLMs) query the model multiple times sequentially -- first to produce intermediate results and then the final answer. However, using these methods, both decoder and model are unaware of potential follow-up prompts, leading to disconnected and undesirably wordy intermediate responses. In this work, we address this issue by proposing prompt sketching, a new prompting paradigm in which an LLM does not only respond by completing a prompt, but by predicting values for multiple variables in a template. This way, sketching grants users more control over the generation process, e.g., by providing a reasoning framework via intermediate instructions, leading to better overall results. The key idea enabling sketching with existing, autoregressive models is to adapt the decoding procedure to also score follow-up instructions during text generation, thus optimizing overall template likelihood in inference. Our experiments show that in a zero-shot setting, prompt sketching outperforms existing, sequential prompting schemes such as direct asking or chain-of-thought on 7 out of 8 LLM benchmarking tasks, including state tracking, arithmetic reasoning, and general question answering. To facilitate future use, we release a number of generic, yet effective sketches applicable to many tasks, and an open source library called dclib, powering our sketch-aware decoders.

==> figures/fig1.tex <==
\begin{figure*}
    \centering
    
    \begin{tikzpicture}[remember picture]
    \node[anchor=center,inner sep=0pt] at (-0.5,-0.5) {\includegraphics[width=0.9\linewidth]{figures/fig1.pdf}};
    \node[anchor=north west,inner sep=0pt] at (3.95,3.4) {
        \tiny{
        \fontsize{5pt}{8}\selectfont
        \cite{kojima_large_2022}
        }
    };
\end{tikzpicture}

    \definecolor{highblue}{RGB}{161,191,249} 
    \sethlcolor{highblue}
    \vspace{-1mm}
    \caption{
        \textit{Prompt Sketching} is multi-part prompting paradigm that allows for more control over the output format and model reasoning process. Only \hl{highlighted} text is generated by the model, where \textbf{\lstinline|THOUGHT|} and \textbf{\lstinline|RESPONSE|} mark the generated (intermediate) outputs.
    }
    \label{fig:main_example}
    \vspace{-3mm}
\end{figure*}
